Critiquing Computing Artifacts through Programming Satirical Python Scripts

Computing artifacts tend to exclude marginalized students, so we must create new methods to critique and change them. We studied the potential for "satirical programming" to critique artifacts as part of culturally responsive computing (CRC) pedagogy. We conducted a one-hour session for three different BPC programs (N=51). We showed an example of a satirical Python script and taught elements of Python to create a script. Our findings suggest this method is a promising CRC pedagogical approach: 50% of marginalized students worked together to create a satirical script, and 80% enjoyed translating their "glitches" into satirical Python scripts.

==> conference_respect012621.tex <==
% \documentclass[conference]{IEEEtran}
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
\usepackage{pgfplots, pgfplotstable}
\usepackage{makecell}
\pgfplotsset{compat=1.18}
\definecolor{A}{HTML}{4DBD05}
\definecolor{B}{HTML}{1FBEB8}
\definecolor{C}{HTML}{0088C9}
\definecolor{D}{HTML}{6563C4}
\definecolor{E}{HTML}{9B45A3}

\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% The following commands add the horizontal rule above the funding agency information
\makeatletter
\renewcommand\footnoterule{%
  \kern-3\p@
  \hrule\@width 1\columnwidth
  \kern2.6\p@}
  \makeatother
  
% If using multiple lines of authors, use \linebreakand to cleanly align author rows
\newcommand{\linebreakand}{%
  \and[\hfill\mbox{}\\\mbox{}\hfill]
}


\begin{document}

\IEEEoverridecommandlockouts
\IEEEpubid{\makebox[\columnwidth]{ XXX-X-XXX-XXXX-6/23/\$31.00~\copyright 2023 IEEE \hfill} \hspace{\columnsep}\makebox[\columnwidth]{ }}


\title{Critiquing Computing Artifacts through Programming Satirical Python Scripts}

\author{\IEEEauthorblockN{Aadarsh Padiyath}
\IEEEauthorblockA{\textit{School of Information} \\
\textit{University of Michigan}\\
Ann Arbor, USA \\
aadarsh@umich.edu}
\and
\IEEEauthorblockN{Tamara Nelson-Fromm}
\IEEEauthorblockA{\textit{School of Engineering} \\
\textit{University of Michigan}\\
Ann Arbor, USA \\
tamaranf@umich.edu}
\and
\IEEEauthorblockN{Barbara Ericson}
\IEEEauthorblockA{\textit{School of Information} \\
\textit{University of Michigan}\\
Ann Arbor, USA \\
barbarer@umich.edu}}


\maketitle

\begin{abstract}
Computing artifacts tend to exclude marginalized students, so we must create new methods to critique and change them. We studied the potential for ``satirical programming" to critique artifacts as part of culturally responsive computing (CRC) pedagogy. We conducted a one-hour session for three different BPC programs (N=51). We showed an example of a satirical Python script and taught elements of Python to create a script. Our findings suggest this method is a promising CRC pedagogical approach: 50\% of marginalized students worked together to create a satirical script, and 80\% enjoyed translating their ``glitches" into satirical Python scripts.\newline
\end{abstract}

\begin{IEEEkeywords}
culturally responsive computing, critical computing education, satirical programming
\end{IEEEkeywords}

\section{Introduction}

In its push to Broaden Participation in Computing (BPC), the computer science (CS) community created several programs focused on increasing access and helping marginalized students succeed in a computing culture that tends to oust them \cite{gilbert2006making}. However, there are increasing calls for these programs to create and center methods for critiquing and changing the culture and its artifacts that left out marginalized students in the first place \cite{vakil2018ethics, ko2020time, guzdial2020cs}. 

Storytelling through satire has the potential to draw attention to particular issues and use wit to expose and ridicule flaws in a system. Many marginalized students have experienced what Dr. Ruha Benjamin calls ``glitches": a breakdown of computing artifacts regarding the intersection of identities and computing that expose systemic biases \cite{benjamin2019race}. Programming satirical scripts of ``glitches" have the unique possibility for marginalized programmers to learn and practice technical programming skills, expose systemic biases in software engineering, as well as reflect and demonstrate how technology intersects and interacts with their identities.

In this exploratory study, we describe the experience of using ``satirical programming" for scaffolding critical reflection of computing artifacts using culturally responsive pedagogy. We piloted this teaching method with majority students of color (N=51) in BPC programs from under-resourced high schools and community colleges in the Midwest region of the United States. We distributed a post-survey to measure reactions to the session and collected the students' Python programs for analysis.

\section{``Satirical Programming"}
In this study, we define the term \textit{``Satirical Programming"} as a programming script that uses satire/comedy to express a social critique, often of systemic biases. For example, when writing the first author's traditionally non-Western name on a word processing document, it frequently will be auto-corrected, but a traditionally Western name will not. In this situation, we can see how auto-correction technology was not designed for names like the first author's. This bias against non-Western names can be shown through a satirical programming script as shown in Figure \ref{fig:autocorrect}.

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{autocorrect.png}
  \caption{A satirical Python script of auto-correct based on the first author's experiences of typing a non-Western name in word processors.}
  \label{fig:autocorrect}
\end{figure}


\section{Description of Practice}

\subsection{Learning Session}

We created a one-hour session outline as a probe for a lecture session in three BPC programs in the American Midwest based on findings from a review of the literature. This probe is inspired by and uses concepts from ``Chapter 4: Teaching CS, Equity, and Justice" and ``Chapter 10: Programming Languages" in \textit{Critically Conscious Computing} \cite{ko2022critically}.

\noindent \textit{Learning Objectives:}

\begin{enumerate}
    \item Students will be able to use variables, print strings, and use the input function in the Python programming language.
    
    \item Students will be able to create a satirical Python script about a ``glitch" they experienced.
    
\end{enumerate}

\noindent \textit{Session Outline:}

\begin{itemize}
    \item (5 mins) Begin the session by discussing rules in social systems, how assumptions are inherent to these rules, and how it translates to the design of software. Support the concept by starting the discussion with assumptions inherent to a context they may be familiar with: college admissions.
    \item (10 mins) Ask students to help brainstorm in groups the many situations in which their identity was not accounted for by software. Scaffold this through thinking about times technology didn't understand them, or through popular things they heard about in the news. As students brainstorm, write these ``glitches" down in a shared space so that everyone can see them.
    \item (5 mins) Explain that software is designed by a specific person or group of people with particular experiences and values. The negative experiences that students have with software are a result of a mismatch of these experiences and values. Additionally, as the group of people that design software is overwhelmingly White and Asian men, the software often ``glitches" when encountering other identities, exposing systemic biases.
    \item (5 mins) Discuss the relationship between rules and computing languages: This includes syntax of strings, variables, and the input and print function in Python as decisions the designer of Python made.
    \item (15 mins) Walk through practice problems for the Python concepts, with a focus on the hidden assumptions of using Python. For example, this can include a discussion of the knowledge barrier of error messages in Python. When omitting a closing quote on a string, the compiler throws the error: ``Syntax Error: EOL while scanning string literal." This information is not accessible to new programmers and contains programmer jargon. This can be connected to the assumptions made by the designer of Python: programmers using Python will be able to understand this message and have enough information to fix the issue.
    \item (15 mins) Ask students to choose a ``glitch" they or their classmates shared, specifically one they would like to discuss or one that impacts themselves. Showcase a personal experience of a ``glitch" turned into a satirical script. Then discuss together how they can tell an interactive story about the experience by using strings, variables, and the input function in Python. They can work together in groups if they like, or they can work by themselves.
    \item (5 mins) Allow students the opportunity to share their creations for everyone to view if they wish to share. Then end the session by bringing assumptions and software back into focus. Discuss the importance of listening to those that are often marginalized, and working with marginalized communities to design software for a world we all belong in.
\end{itemize}

\subsection{Sites}

We conducted this study with three BPC Summer programs for high school or community college students entering college computing programs: 
Wolverine Pathways (WP)\footnote{https://wolverinepathways.umich.edu/}, LSAMP NxtGEN STEM Scholars Program (LSAMP)\footnote{https://www.milsamp.org/programs/}, and Community College Summer Institute (CCSI)\footnote{https://www.si.umich.edu/programs/bachelor-science-information/new-transfers/umsi-community-college-summer-institute}. A breakdown of reported student demographics is displayed in Table \ref{tab:demo}. Each site had one instructor (the first author) use the session outline described above.

\begin{table}[ht]
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline
        \textbf{Program} & WP & LSAMP & CCSI \\
        % \textbf{Program} & Anon1 & Anon2 & Anon3 \\
        \hline
        \textbf{\# of Participants} & 15 & 13 & 23 \\
        \hline
        \textbf{Gender Ratios} & \makecell{60\% Women\\40\% Men} & \makecell{38\% Women\\62\% Men} & \makecell{57\% Women\\43\% Men} \\
        \hline
        \textbf{URM Ratio} & 95\% & 100\% & 87\% \\
        \hline
        \textbf{Delivery} & Zoom & Zoom & In-person \\
        \hline
    \end{tabular}
    \newline
    \caption{Demographic breakdowns of each site retrieved by University of Michigan's DEI Office.}
    \label{tab:demo}
\end{table}

\subsection{Data Collection}

We distributed an online survey after completing the session. The survey was sent to the email address provided to the program right after the session. This survey context was modified to fit this study from an NCWIT E-Textiles Teacher Workshop Experience Survey that evaluated teachers' experience with an introductory computing workshop, including enjoyment \cite{ncwitetextileteacherworkshopurvey}.

The course sessions used the interactive open-source e-book system, Runestone, as a programming environment \cite{ericson2020runestone}. Students were presented with a Runestone assignment page containing practice problems relating to the technical concepts in class, as well as space to write their satirical script. Coding logs and satirical Python scripts were collected through this system. Specifically, it collected submissions to the Python compiler when attempting to run written code.

\section{Positionality}

Key to culturally responsive computing pedagogy is the need for cultural competence of educators \cite{washington2020twice}. As this requires serious and continuous reflection of an educator's identities and motivations, I share how my experiences led to and influenced this study. Several experiences of my identity clashing with computing culture and its artifacts led me to rejecting the harmful dominant ideologies of computing culture and heavily informed this work. I do this work to critique and change computing culture and its artifacts to create futures we can live and belong in. As a \textit{Desi} (South Asian) man, my identity stands within a prominent subgroup of the dominant culture of computing: cis-gendered White and Asian men. Although my queer identity is certainly not the norm within this dominant culture, there is still a challenge and gap in research in bringing my identity and positionality to this context. Many White lecturers within the dominant culture of education struggle to engage in discussions of critical counternarratives, race, and power \cite{johnson2011road, porfilio2011guiding, bolgatz2005teachers}. Thus I approach this context with humility and care.

\section{Experiences and Reflections}

\subsection{Student Artifacts and Reactions}

In analyzing students' (N=51) experiences, we found that several students exhibited existing or newfound recognition of ``glitches" that revealed systemic biases encoded in technologies. Students worked in groups to discuss and share ``glitches" they have experienced, submitting a total of 23 ``glitches." Repeating themes in students' written experiences included non-traditional names and auto-correct (8/23; 35\%); light-skin bias in cameras/camera filters (4/23; 17\%); White hairstyle bias in search results and video games (3/23; 13\%); and restrictive or automatic categorizations (4/23; 17\%). Examples of student responses grouped by these themes are displayed in Table \ref{tab:glitches}.

\begin{table}[h]
    \centering
    \begin{tabular}{|p{0.3\linewidth} | p{0.6\linewidth}|}
    \hline
        Non-traditional names and auto-correct & When I search my name in a
search engine, the meaning always
comes up as ``tree" when my
parents always tells me it means
god's message. \\
\cline{2-2}
         & When I type my name it can
auto-correct to a different name,
and many people mishear me
when I say it to them, which leads
to them recording it wrong. \\
        \hline
        Light-skin bias in cameras/camera filters & My friend who is of darker skin
color than mine, was having
issues getting software to
recognize her face and pattern it
correctly \\
\cline{2-2}
         & Often times, photo editing
software or phones will tell darker
skinned people to turn up
exposure or won't recognize their
face at all\\
        \hline
        White hairstyle bias in search results and video games & In most video games, most
of the preset game hairstyles are
straight or only have Euro-centric
hairstyles.\\
\cline{2-2}
         & When looking up ideas, such as
makeup, hairstyles or outfit ideas
the search engine assumes our
race and we never see people of
color.\\
        \hline
        Restrictive or automatic categorizations & Automatic gender
assumption cookie when online shopping it
automatically picks a gender
specific clothing. \\
\cline{2-2}
         & Race options on
applications: Being mixed raced and not
knowing what option to choose, or
the reason for needing to specify
race on an application at all\\
        \hline
    \end{tabular}
    \newline
    \caption{Example student responses of ``glitches" in their interactions with technology grouped by repeating themes.}
    \label{tab:glitches}
\end{table}

Many students were able to translate these ``glitches" into critiques in the form of satirical Python scripts. 
One student created a satirical critique of their experience with a light-skinned bias in cameras and camera filters. The script, shown in Figure \ref{fig:camera}, asks if a user wishes to take a photo. If the user does, it then asks if the user is light or dark skinned. If they are light-skinned, the script prints ``Nice photo! Lookin pretty normal to me!" However, if they are dark-skinned, the script prints, ``Oh whoops! You might want to wipe off your camera lens to get a clearer picture."


\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{camera.png}
  \caption{A satirical Python script of using a camera based on a student's experience with camera filters.}
  \label{fig:camera}
\end{figure}

Another student translated their experience with White bias in recommendations for hairstyles into a satirical critique. The script first notes that it will provide a hairstyle recommendation based on someone's name. The script then asks the user for a name. It compares the name against 5 common Western White women names. If the name was one of those five names, it recommended ``Hair in messy bun." Otherwise, for all other names, it recommends ``Cornrows."

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{hairstyles.png}
  \caption{A satirical Python script of hairstyle recommendations based on a student's experience with online search results.}
  \label{fig:hairstyle}
\end{figure}


Students also worked in groups or by themselves to submit a total of 34 Python scripts. In 7 out of 34 scripts (21\%), students were able to identify a ``glitch" in their experiences with technology and communicate a satirical critique of the experience in a Python script. Many students (10/34; 29\%) created the beginnings of a critique through their script, however, the objective of their script was unclear or missing. For example, the intention of the script in Figure \ref{fig:pronouns} is unclear. The student could be making a statement about many gender and pronoun related issues regarding their intersections with technology, such as a lack of fluidity or intersections in options (such as they/she), a lack of neopronoun options (such as xe/xem), and more. However, this ambiguity reduces the ability for the student to communicate a specific and clear critique with this script.

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{pronounschecker.png}
  \caption{A Python script to validate pronoun options.}
  \label{fig:pronouns}
\end{figure}

In 17 out of the 34 Python scripts, the students chose to not create a satirical critique, but rather express themselves through creating an interactive script. For example, a student created a script for ordering a sandwich from Jimmy John's.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{jimmyjohns.png}
%   \caption{A Python script to order a sandwich from Jimmy John's.}
%   \label{fig:jimmy}
% \end{figure}

Students' reactions to the session were very positive. Based on the post-survey (n=25/51, 49\% response rate), 80\% of students responded positively (4/5 - ``I liked it," or 5/5 - ``I loved it") to the session overall. Figure \ref{fig:likert_questions} displays the distribution of the reactions to the session and its parts. A majority of students ``liked" or ``loved" every part of the session, including the session overall.

\begin{figure}
\begin{tikzpicture}
\pgfplotsset{%
    width=.7\linewidth,
    height=7.5cm
}
\begin{axis}[
    xbar,
    x axis line style = { opacity = 0 },
    hide x axis,
    tickwidth         = 0pt,
    bar width = 6pt,
    enlarge y limits  = 0.15,
    enlarge x limits  = 0.08,
    symbolic y coords = {Writing Stories,Learning Programming,Brainstorming ``Glitches",Session Overall},
    ytick=data,
    nodes near coords,
    legend style={at={(0.8,1.03)},anchor=south east},
    legend columns=3,
    table/col sep=comma
]
\addplot[color=A, fill=A] 
	coordinates {(0,Session Overall) (0,Brainstorming ``Glitches")
		 (0,Learning Programming) (0,Writing Stories)};
\addplot[color=B, fill=B]  
	coordinates {(1,Session Overall) (3,Brainstorming ``Glitches")
		 (0,Learning Programming) (1,Writing Stories)};
\addplot[color=C, fill=C]  
	coordinates {(4,Session Overall) (5,Brainstorming ``Glitches")
		 (7,Learning Programming) (8,Writing Stories)};
\addplot[color=D, fill=D]  
	coordinates {(14,Session Overall) (14,Brainstorming ``Glitches")
		 (12,Learning Programming) (12,Writing Stories)};
\addplot[color=E, fill=E]  
	coordinates {(6,Session Overall) (3,Brainstorming ``Glitches")
		 (6,Learning Programming) (4,Writing Stories)};
\legend{I hated it,I disliked it,It was ok,I liked it,I loved it}
\end{axis}
\end{tikzpicture}
\caption{Distribution of responses (N=25) to the post-survey containing 5-point Likert scale questions regarding reactions to the session and its parts.}
\label{fig:likert_questions}
\end{figure}

In response to the open-ended question in the post-survey, \textit{Please tell us about your experience during the session. What was fun, what was challenging, what was frustrating?}, a majority of students (n=10/18; 56\%) mentioned appreciating the critical approach to Python. Several students noted having fun translating their experiences into a Python script, writing specifically that this challenge kept the learning experience fun (12/18; 67\%). Several students mentioned the experience was challenging yet fun and engaging (7/18; 39\%).


\subsection{Instructor Reflections}
Throughout the design and execution process, I actively worked to hold myself accountable for any possible harm caused by this research. This included a thorough self-reflection of my values and motivation regarding this project and my positionality; seeking out minoritized individuals from similar backgrounds of the participants whom I trusted to give me honest criticism of this study; explicitly asking for pushback if students felt uncomfortable or were apprehensive throughout the session; vigilantly observing in-person student reactions for uneasiness or wariness throughout the sessions; and planning for divergences from the session plans if necessary. I recommend this preparation and vigilance for those looking to adopt this method, as this approach is not suitable for all contexts.

In the design of this session, we expected difficulties in both identifying ``glitches" and translating them into satirical programs. Most students recognized ``glitches" in their experiences with technology, however, many students still had difficulties in translating their experiences into a focused critique within a Python script. This was challenging, as there were several groups of students working on Python scripts, but only one instructor to assist them. When students had difficulties in proposing a satirical critique and asked for assistance, we focused on identifying the systemic biases the ``glitch" exposes. Then, we discussed what experiencing the ``glitch" felt like, and what seemed absurd or stupid about it. Next, we urged the students to re-create that absurd experience using Python to communicate their satirical critique.

Although we stressed ``creativity first, programming second" throughout the session, several students were frustrated when their code had errors. In assisting these students, we reminded the students of the unhelpful error messages the creator of Python designed. This shifted the blame of not understanding Python from the students to the designers of Python.




\section{Conclusion}

In this study we explored a pedagogical method for identifying systemic biases in computing artifacts and creating satirical critiques of our experiences. Our findings show that this method was promising for culturally responsive computing classes in that students enjoyed the session beyond solely the technical content knowledge and enabled several students to understand ``glitches" and create satirical scripts that reflects how their identities interact with technologies. As students lives increasingly intersect with technology, minoritized youth deserve to understand how systemic biases manifest in software and how to push forward from oppressive experiences. Satirical programming scripts are a unique rhetorical device positioned to turn these oppressive experiences with technology into constructive and powerful critiques about the necessity for diversity, equity, and inclusion in software development.

\subsection{Limitations}

There are several key limitations to this study. One limitation is the context in which the project was given: this study was conducted with a relatively small number of participants, with a specific demographic of participants, at one school, in one institution and in one country. The response rate for the post-survey was low, possibly due to the programs sending the survey to parents' email addresses. Students may have realized I was a researcher and responded positively to the survey to please me. Additionally, this was the first author's first teaching experience. Instructors with more teaching experience may find this method easier to employ.

\subsection{Future Work}

Future work can address these limitations and explore the pedagogical methods and metaphors used in this study. For example, more research is needed in employing this method in classes with diverse demographics. The use of satire in programming with diverse classes could support cross-cultural understanding, or alternatively could place undue burden and hypervisibility on minoritized students.



% \section*{Acknowledgment}
% Acknowledgements anonymized.
% Thanks to Mark Guzdial and Patricia Garcia for valuable feedback. Thanks to Tamara Nelson-Fromm for assisting in qualitative coding.


\bibliographystyle{IEEEtran}
\bibliography{sources.bib}

\end{document}

